Minimal Mechanisms of Microtubule Length Regulation in Living Cells

The microtubule cytoskeleton is responsible for sustained, long-range intracellular transport of mRNAs, proteins, and organelles in neurons. Neuronal microtubules must be stable enough to ensure reliable transport, but they also undergo dynamic instability, as their plus and minus ends continuously switch between growth and shrinking. This process allows for continuous rebuilding of the cytoskeleton and for flexibility in injury settings. Motivated by \textit{in vivo} experimental data on microtubule behavior in \textit{Drosophila} neurons, we propose a mathematical model of dendritic microtubule dynamics, with a focus on understanding microtubule length, velocity, and state-duration distributions. We find that limitations on microtubule growth phases are needed for realistic dynamics, but the type of limiting mechanism leads to qualitatively different responses to plausible experimental perturbations. We therefore propose and investigate two minimally-complex length-limiting factors: limitation due to resource (tubulin) constraints and limitation due to catastrophe of large-length microtubules. We combine simulations of a detailed stochastic model with steady-state analysis of a mean-field ordinary differential equations model to map out qualitatively distinct parameter regimes. This provides a basis for predicting changes in microtubule dynamics, tubulin allocation, and the turnover rate of tubulin within microtubules in different experimental environments.

==> preamble.tex <==
%\textwidth = 6 in \textheight = 8.5 in \oddsidemargin = 0.0 in
%\evensidemargin = 0.0 in \topmargin = 0.0 in \headheight = 0.0 in
%\headsep = 0.25 in
%\parskip = 0.1 in
%\parindent = 0.0 in

\usepackage[margin=3cm]{geometry}
\usepackage{caption}
\usepackage{subcaption}
\captionsetup{font=small} 
\usepackage{graphicx}%
\usepackage{multirow}%
\usepackage{amsmath,amssymb,amsfonts}%
\usepackage{amsthm}%
\usepackage{mathrsfs}%
\usepackage{latexsym}%
\usepackage{mathtools}%
\usepackage[title]{appendix}%
\usepackage{xcolor}%
\usepackage{color,cancel}
%\usepackage[normalem]{ulem}
\usepackage{textcomp}%
\usepackage{manyfoot}%
%\usepackage{fullpage}
\usepackage[utf8]{inputenc}
\usepackage{listings}%

\usepackage{tocloft}
\usepackage{authblk}
\usepackage{lipsum}
\usepackage{wrapfig}
\usepackage{enumerate}
\usepackage{soul}
\usepackage{chemarrow}


% Table packages
\usepackage{booktabs}%
\usepackage{multicol}
\usepackage{multirow}
\usepackage[math]{cellspace}
\cellspacetoplimit 4pt
\cellspacebottomlimit 4pt
%\setlength{\tabcolsep}{6pt} % Default value: 6pt
%\renewcommand{\arraystretch}{1.15} % Default value: 1
%\usepackage{ctable}
%\usepackage[table]{xcolor}
%\usepackage{colortbl}
%\usepackage{tabularx}

\usepackage{algorithm}%
\usepackage{algorithmicx}%
\usepackage{algpseudocode}%
\usepackage{listings}%
\usepackage{units}
\usepackage{verbatim}
\usepackage{fancyvrb}
\fvset{fontsize=\normalsize}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\usepackage[T1]{fontenc}
\usepackage[sc]{mathpazo}
\linespread{1.1}         % Palatino needs more leading (space between lines)
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\setkeys{Gin}{width=\linewidth,totalheight=\textheight,keepaspectratio}
\newcommand{\textblue}[1]{\textcolor{blue}{{#1}}}

\usepackage{hyperref}
\hypersetup{
	hidelinks = true
}
%\usepackage{floatflt}
%\usepackage{stmaryrd}



\renewcommand{\d}{\mathrm{d}}
\newcommand{\rbb}{\mathbb{R}}
\newcommand{\ep}{\epsilon}
\newcommand{\f}{\varphi}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\suchthat}{\, : \,}
\newcommand{\given}{\, | \,}
\newcommand{\with}{\, ; \,}
\newcommand{\wtilde}[1]{\widetilde{#1}}

\newtheorem{theorem}{Theorem}[section]
\newtheorem{proposition}[theorem]{Proposition}
\newtheorem{definition}[theorem]{Definition}
\newtheorem{corollary}[theorem]{Corollary}
\newtheorem{lemma}[theorem]{Lemma}
\newtheorem{remark}[theorem]{Remark}

\newcommand{\lambdags}{\lambda_{\mathrm{g} \to \mathrm{s}}}
\newcommand{\lambdasg}{\lambda_{\mathrm{s} \to \mathrm{g}}}
\newcommand{\rescue}{\lambda_\mathrm{rescue}}
\newcommand{\cat}{\lambda_\mathrm{cat}}
\newcommand{\catform}{\phi}
\newcommand{\catf}{\phi}
\newcommand{\mtzero}{\psi}
\newcommand{\Tnd}{\widetilde{T}}
\newcommand{\lchar}{\ell_\mathrm{char}}
\newcommand{\lcrit}{\ell_\mathrm{crit}}
\newcommand{\Lchar}{L_\mathrm{char}}
\newcommand{\Lcrit}{L_\mathrm{crit}}
\newcommand{\lambdamin}{\lambda_\mathrm{min}}
\newcommand{\ndlambdamin}{\widetilde{\lambda}_\mathrm{min}}
\newcommand{\tchar}{t_\mathrm{char}}
\newcommand{\vgmax}{v_g^{\mathrm{max}}}
\newcommand{\vgavg}{\overline{v}_g}
\newcommand{\vsmax}{v_s^{\mathrm{max}}}
\newcommand{\vsavg}{\overline{v}_s}
\newcommand{\vsind}{\overline{v}_s}
\newcommand{\vspop}{\langle v_s \rangle}
\newcommand{\taugavg}{\overline{\tau}_g}
\newcommand{\tausavg}{\overline{\tau}_s}
\newcommand{\tauspop}{\langle \tau_s \rangle}
\newcommand{\mtavg}{\overline{L}}
\newcommand{\micron}{\mu \mathrm{m}}
\newcommand{\domain}{\mathcal{O}}


